TimeSuite: Improving MLLMs for Long Video Understanding via Grounded Tuning

Multimodal Large Language Models (MLLMs) have demonstrated impressive performance in short video understanding. However, understanding long-form videos still remains challenging for MLLMs. This paper proposes TimeSuite, a collection of new designs to adapt the existing short-form video MLLMs for long video understanding, including a simple yet efficient framework to process long video sequence, a high-quality video dataset for grounded tuning of MLLMs, and a carefully-designed instruction tuning task to explicitly incorporate the grounding supervision in the traditional QA format. Specifically, based on VideoChat, we propose our long-video MLLM, coined as VideoChat-T, by implementing a token shuffling to compress long video tokens and introducing Temporal Adaptive Position Encoding (TAPE) to enhance the temporal awareness of visual representation. Meanwhile, we introduce the TimePro, a comprehensive grounding-centric instruction tuning dataset composed of 9 tasks and 349k high-quality grounded annotations. Notably, we design a new instruction tuning task type, called Temporal Grounded Caption, to peform detailed video descriptions with the corresponding time stamps prediction. This explicit temporal location prediction will guide MLLM to correctly attend on the visual content when generating description, and thus reduce the hallucination risk caused by the LLMs. Experimental results demonstrate that our TimeSuite provides a successful solution to enhance the long video understanding capability of short-form MLLM, achieving improvement of 5.6% and 6.8% on the benchmarks of Egoschema and VideoMME, respectively. In addition, VideoChat-T exhibits robust zero-shot temporal grounding capabilities, significantly outperforming the existing state-of-the-art MLLMs. After fine-tuning, it performs on par with the traditional supervised expert models.

==> algorithm/token_shuffle.tex <==
\lstset{language=Python,
        basicstyle=\tiny\ttfamily,
        keywordstyle=\color{blue},
        commentstyle=\color{green},
        stringstyle=\color{red},
        numbers=none,
        showstringspaces=false,
        breaklines=true,
        tabsize=4,
        lineskip=-1em,
}



\begin{algorithm}
\caption{Example Algorithm}
\begin{algorithmic}[]

\STATE Efficient Initialization
\begin{lstlisting}
new_mistral_weight = self.mistral_proj.weight.data.repeat(1, self.token_merge_len)
self.merge_proj.weight.data = new_mistral_weight / self.token_merge_len
self.merge_proj.bias.data = self.mistral_proj.bias.data
\end{lstlisting}

\STATE Token Shuffle
\begin{lstlisting}
batch_size, token_len, token_dim = video_embeds.shape
video_embeds = video_embeds.view(batch_size, token_len//self.token_merge_len, \\
                self.token_merge_len * token_dim)
video_embeds = self.merge_proj(video_embeds)
\end{lstlisting}

\end{algorithmic}
\end{algorithm}

==> tables/old/ablation_tokenshuffle.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3pt}
\resizebox{0.6\textwidth}{!}{


\begin{tabular}{l|cccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \textbf{Egoschema} & \textbf{VideoMME} & \textbf{Charades-STA} & \textbf{QVHighlights} \\
                                & Full               & w/o subs          & R@1 IOU=0.5           & Hit@1                 \\ \hline

\rowcolor{gray!15}
VideoChat-T(Ours)               & 60.0               & 46.3              & 48.7                  & 54.1                  \\

r/w pooling                     & 59.8                  & 44.8                 & 40.3                     &            47.3           \\

r/w cluetering                  & 59.5                  & 45.0                 & 39.8                     & 40.1                     \\

w/o init                        & 57.4                  & 43.4                 & 42.0                     & 53.9                     \\

\hline
\end{tabular}



}


\caption{
% 表4. Token Shuffle 相关设计的消融实验。 其中r/w指的是将Token Shuffle替换成对应的组件，w/o init指的是不使用高效初始化方法。
Performance results of the ablation study on the Token Shuffle. Here, r/w refers to replacing Token Shuffle with the other component, and w/o init refers to removing the efficient initialization.
}


\end{table}

==> tables/old/ablition_adapter.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3pt}
\resizebox{0.6\textwidth}{!}{


\begin{tabular}{l|cccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \textbf{Egoschema} & \textbf{VideoMME} & \textbf{Charades-STA} & \textbf{QVHighlights} \\
                                & Full               & w/o subs          & R@1 IOU=0.5           & Hit@1                 \\ \hline

\rowcolor{gray!15}
VideoChat-T(Ours)               & 60.0               & 46.3              & 48.7                  & 54.1                  \\
w/o TAPE            & 59.1               & 45.9              & 47.1                  & 50.4                  \\

w/o frz                    & 59.0                  & 45.2                 & 52.4                     & 53.7                     \\
\hline
\end{tabular}



}


\caption{
% 表3. Temporal Adapter相关设计的消融实验。其中w/o adapter指不使用我们提出的Temperal Adapter，w/o frz指不使用在第一个epoch冻结Temporal Adapter的训练方法。
Performance results of the ablation study on the TAPE Adapter. Here, w/o adapter refers to removing our proposed TAPE Adapter, and w/o frz refers to not using the training method where the TAPE Adapter is frozen during the first epoch.
}


\end{table}
